Hand Me Your PIN! Inferring ATM PINs of Users Typing with a Covered Hand

Automated Teller Machines (ATMs) represent the most used system for withdrawing cash. The European Central Bank reported more than 11 billion cash withdrawals and loading/unloading transactions on the European ATMs in 2019. Although ATMs have undergone various technological evolutions, Personal Identification Numbers (PINs) are still the most common authentication method for these devices. Unfortunately, the PIN mechanism is vulnerable to shoulder-surfing attacks performed via hidden cameras installed near the ATM to catch the PIN pad. To overcome this problem, people get used to covering the typing hand with the other hand. While such users probably believe this behavior is safe enough to protect against mentioned attacks, there is no clear assessment of this countermeasure in the scientific literature. This paper proposes a novel attack to reconstruct PINs entered by victims covering the typing hand with the other hand. We consider the setting where the attacker can access an ATM PIN pad of the same brand/model as the target one. Afterward, the attacker uses that model to infer the digits pressed by the victim while entering the PIN. Our attack owes its success to a carefully selected deep learning architecture that can infer the PIN from the typing hand position and movements. We run a detailed experimental analysis including 58 users. With our approach, we can guess 30% of the 5-digit PINs within three attempts -- the ones usually allowed by ATM before blocking the card. We also conducted a survey with 78 users that managed to reach an accuracy of only 7.92% on average for the same setting. Finally, we evaluate a shielding countermeasure that proved to be rather inefficient unless the whole keypad is shielded.

==> sections/Background.tex <==

The proposed attack relies on a machine learning hand and finger tracking strategy to overcome detecting hand movements regardless of partial occlusion.
During the last years, the tracking and classification of hand and finger poses/motion have been extensively investigated in computer vision due to their application to different fields ranging from Human-Computer Interaction (HCI)~\cite{poz14:hand_robot} to training and rehabilitation in medical application~\cite{Boa09:hand}. 
For this purpose, different types of sensors have been used, like the standard RGB camera~\cite{wa11:hand_gesture,Zab09:hand_gesture}, structured-light depth sensors, 3D Time-of-Flight scanners~\cite{Zen15:TofSL}, and infrared tracking devices~\cite{Vys20:leapmotion_hand}, to mention some of them. 

The traditional pipeline for hand-pose tracking and classification can be summarized by the following steps, reported in the diagram of Figure~\ref{fig:hand}.

\begin{figure}[htp]
\centering 
\includegraphics[width=0.9\linewidth]{figures/hand_gest.png}
\caption{Hand tracking and classification diagram.}
\label{fig:hand}
\end{figure}

The input data are sequences of two-dimensional frames corresponding to the acquired signals from RGB or depth cameras. The localization unit identifies the hand's presence and its centroid for each frame to focus the analysis on the interesting region only. This operation allows excluding other visual elements from the classification process, improving the final accuracy. The hand shape is estimated at the following stage via segmentation algorithms that extract its silhouette from the input frame. In these initial phases, 3D devices have allowed enhancing the performances of traditional approaches~\cite{Kha19:handRGBRGBD} since hand segmentation from depth data proves to be more robust and less conditioned by illumination noise (object boundaries can be identified). Following this initial pre-processing, a set of hand-pose features need to be computed, ranging from morphological operators (like skinning or skeletonization) \cite{DeS16:hand_skeleton} to gradients and local visual features.
This permits fitting the acquired data to a predefined model (since the standard articulation and the appearance of hands are fixed and known in advance), enhancing the final accuracy of the last classification stage~\cite{Kre13:finger_tracking}. In dynamic classification, these steps are integrated into a time-dependent framework where the correlation among different frames is exploited to obtain a more accurate localization and modeling.

Although the schemes based on 3D sensors rank among the top state-of-the-art strategies for hand tracking and gesture classification, the recent development of deep learning (DL) has improved the detection performances on standard RGB cameras too~\cite{Zim17:hand}. Indeed, the processing architectures can be taught to overcome adversarial conditions like acquisition noise, bad illumination, and heterogeneity in the gesture alphabet. Moreover, the different phases of traditional pipelines can be merged into integrated schemes where the different units can be jointly optimized~\cite{Dad18:hgrnet}.

Among the first approaches that are worth mentioning, we mention the solutions based on Convolutional Neural Networks (CNNs)~\cite{Kim08:cnn_hand,Mol15:3dcnn_hand}, where a hierarchically-decreasing pipeline of the convolutional layers are used to generate a set of shape features that are finally classified by the last fully-connected stages into a static hand pose.
Some other solutions combine traditional image pre-processing steps aimed at cleaning and refining the image quality before classifying the resulting image with the DL detection architecture\cite{Aga19:hand_cnn}. In other strategies, the use of contexts allows the network to generate separate manifolds in the training phase~\cite{Hak19:hand_context}.
To identify dynamic hand gesture, more recent solutions combines the traditional CNN schemes with Recurrent Neural Networks (RNN)~\cite{Lai18:cnnrnn} and Long-Short Time Memory (LSTM)~\cite{Nun18:lstm_hand,Zha17:lstm} modules. Indeed, temporal information can be effectively exploited by segmenting the video sequence into frames~\cite{wang2016temporal}, which are lately classified.
This result was possible thanks to the availability of large datasets derived from large ego-motion databases, by the development of enhanced data augmentation~\cite{Isl19:hand_augmentation}, and synthesis strategies~\cite{GANeratedHands_CVPR2018} (e.g., based on Generative Adversarial Networks or GANs), which enabled augmenting the amount of data in the training process.

In this work, we are going to focus on the approaches based on traditional 2D video sensors~\cite{wa11:hand_gesture,Zab09:hand_gesture} since the designed attack needs to rely on cheap and easily-concealable video sensing equipment, and standard RGB cameras mostly fit these requirements.
Although hand tracking and gesture recognition research topics have reached some maturity in the computer vision field, most proposed solutions are intended for HCI applications. These solutions imply a collaborative user that interacts with the camera and adapts the hand pose to facilitate the detection. Eventual occlusions and noise may be charged to accidental movements or environmental factors. 

Nevertheless, there are still some adversarial conditions that are worth to be investigated in this detection, such as non-ideal camera positions~\cite{Miao17:rec3D} and focus problems~\cite{Nar18:focus_hand}.
We consider a new adversarial scenario where the user deliberately hides the hand while entering a number on a PIN pad.
This makes the gesture detection task more challenging since the visual information can be highly compromised, and previous solutions prove unable to detect them.





